Universal Streaming of Subset Norms

Most known algorithms in the streaming model of computation aim to approximate a single function such as an $\ell_p$-norm. In 2009, Nelson [\url{https://sublinear.info}, Open Problem 30] asked if it possible to design \emph{universal algorithms}, that simultaneously approximate multiple functions of the stream. In this paper we answer the question of Nelson for the class of \emph{subset $\ell_0$-norms} in the insertion-only frequency-vector model. Given a family of subsets $\mathcal{S}\subset 2^{[n]}$, we provide a single streaming algorithm that can $(1\pm \epsilon)$-approximate the subset-norm for every $S\in\mathcal{S}$. Here, the subset-$\ell_p$-norm of $v\in \mathbb{R}^n$ with respect to set $S\subseteq [n]$ is the $\ell_p$-norm of vector $v_{|S}$ (which denotes restricting $v$ to $S$, by zeroing all other coordinates). Our main result is a near-tight characterization of the space complexity of every family $\mathcal{S}\subset 2^{[n]}$ of subset-$\ell_0$-norms in insertion-only streams, expressed in terms of the "heavy-hitter dimension" of $\mathcal{S}$, a new combinatorial quantity that is related to the VC-dimension of $\mathcal{S}$. In contrast, we show that the more general turnstile and sliding-window models require a much larger space usage. All these results easily extend to $\ell_1$. In addition, we design algorithms for two other subset-$\ell_p$-norm variants. These can be compared to the Priority Sampling algorithm of Duffield, Lund and Thorup [JACM 2007], which achieves additive approximation $\epsilon\|{v}\|$ for all possible subsets ($\mathcal{S}=2^{[n]}$) in the entry-wise update model. One of our algorithms extends this algorithm to handle turnstile updates, and another one achieves multiplicative approximation given a family $\mathcal{S}$.

==> results.tex <==
In this paper, we make several contributions.
\begin{itemize}
\item A complete characterization of additive-error subset-norm: we provide an efficient streaming algorithm that makes a pass over a stream of updates to some vector $v\in \RR^n$ and stores a nearly optimal-sized summary. From this summary, one can query any subset $S\subset[n]$, the algorithm is able to output an estimate that approximates $(\sum_{i\in S}|v_i|^p)^{1/p}$ up to additive error $\epsilon (\sum_{i\in [n]}|v_i|^p))^{1/p}$;
We show that our algorithm is space optimal.
\item Weight subset-norm: our algorithm can also be generalized to approximate arbitrarily weighted norm: $(\sum_{i\in S}w_i|v_i|^p)^{1/p}$. Our algorithm makes a pass of the stream without the information of the weights $w_i$;
\item A complete characterization of multiplicative approximation of subset-$F_0$: suppose for now we are given a set family $\cF\subset 2^{[n]}$, we want a summary over an insertion-only stream of a vector $v\in \RR^n$ and at the end we would like obtain an $(1\pm\epsilon)$ approximation to $\sum_{i\in S}\mathbb{I}(v_i\neq0)$. 
We show that the space complexity of this problem is characterized by a notation of ``heavy hitter dimension'' of the set system $\cF$, which characterizes the maximum number of ``singleton''s (the only coordinate of $v$ that is contained in some set) possible for all vector $v$.
We show that heavy hitter dimension is a strict upper bound of the VC dimension of the set system.
\end{itemize}

Link to the three theorems.
Move Section 3 to the beginning. 
Theorem numbering with sections.



\textbf{TODO}: Main contribution is multiplicative approximation.
